Pushing the Limits of Low-Resource Morphological Inflection

Recent years have seen exceptional strides in the task of automatic morphological inflection generation. However, for a long tail of languages the necessary resources are hard to come by, and state-of-the-art neural methods that work well under higher resource settings perform poorly in the face of a paucity of data. In response, we propose a battery of improvements that greatly improve performance under such low-resource conditions. First, we present a novel two-step attention architecture for the inflection decoder. In addition, we investigate the effects of cross-lingual transfer from single and multiple languages, as well as monolingual data hallucination. The macro-averaged accuracy of our models outperforms the state-of-the-art by 15 percentage points. Also, we identify the crucial factors for success with cross-lingual transfer for morphological inflection: typological similarity and a common representation across languages.

==> data.tex <==
\section{Data}
\label{sec:data}

Mention the SIGMORPHON challenges.
Data come form Unimorph.

Basic statistics from sigmorphon 2019, task 1: 
43 test languages,
99 language pairs
low-resource languages typically have 100 examples for training, plus 50-100 (or in very few cases, 1000) dev examples for dev.
The high-resource pairs typically have~10.000 training instances.



==> figures/greekexample.tex <==
\begin{figure}
    \centering
    \begin{tabular}{c@{}c}
        \includegraphics[scale=.5]{figures/char.png} & \includegraphics[scale=.5]{figures/tag.png} \\
        a) Character Attention & b) Tag Attention \\
        (bottom: lemma) & (bottom: tags)
    \end{tabular}
    \caption{Attention visualization example from Greek.}
    \label{fig:greekexample}
\end{figure}

==> figures/greekngram.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=.5]{figures/greek_n_gram_prob.png}
    \caption{Greek bigram character probabilities for $p(\cdot \vert \epsilon)$. The distribution over the hallucinated data matches the real distribution match better than the training one (blue bars). \an{plot the difference to the true distribution}}
    \label{fig:greekngram}
\end{figure}

==> figures/kazakhexample.tex <==
\begin{figure}
    \centering
    \begin{tabular}{c@{}c}
        \includegraphics[scale=.3]{figures/kazakhchar.png} & \includegraphics[scale=.3]{figures/kazakhtag.png} \\
        a) Character Attention & b) Tag Attention \\
        (bottom: lemma) & (bottom: tags)
    \end{tabular}
    \caption{Attention visualization example from Kazakh.}
    \label{fig:kazakhexample}
\end{figure}

==> new-results2.tex <==
\begin{table}[ht]
\centering
\tiny
\begin{tabular}{cccccccc}
\toprule
L1 & L2 & L1+L2 & $+\mathcal{L}_l$ & $+\mathcal{H}$ & $+\mathcal{L}_l+\mathcal{H}$ & $\mathcal{H}$ \\ \midrule
russian & \multirow{1}{*}[-.4em]{old} &  40 &  39 &  39 &  \textbf{64} &  \multirow{4}{*}{57.3$\pm$1.5} \\ 
polish & \multirow{1}{*}[-.5em]{church} &  41 &  41 & 59 &  58 &  \\ 
bulgarian & \multirow{2}{*}{slavonic} &  38 &  42 &  44 &  56  \\
all & & 41 & 42 & \textbf{64} & 56 & \\ \midrule
\ifaclfinal
irish & \multirow{4}{*}{old irish} &  2 &  4 &  \textbf{12} &  2 &  \multirow{4}{*}{6$\pm$2} \\ 
belarusian & &  10 & 10 & 10 &  6 &  \\
welsh &  &  4 &  6 & 10 &  6 &   \\ 
all & & 4 & 4 & 8 & 6 & \\ \midrule
\fi
sanskrit & \multirow{3}{*}{pashto} &  20 &  16 &  46 &  44 &  \multirow{3}{*}{46.5$\pm$3.5}  \\ 
persian & &  36 &  28 &  39 & 48 &  \\ 
all & & 29 & 30 & 46 & \textbf{49} & \\ \midrule
welsh & \multirow{2}{*}[-.6em]{scottish} &  46 &  34 &  64 & 64 &  \multirow{4}{*}{58$\pm$2}  \\ 
irish & &  58 &  62 &  \textbf{68} &  66 &   \\ 
latvian & \multirow{2}{*}[.6em]{gaelic}  &  58 &  36 &  58 & 66 &   \\ 
all & & 60 & 64 & 62 & 66 & \\ \midrule
bashkir & \multirow{4}{*}{tatar} &  67 &  64 &  73 &  69 &  \multirow{4}{*}{73$\pm$4.6} \\ 
uzbek &  &  55 &  45 &  67 & 72 & \\ 
turkish &  &  81 &  79 &  82 &  75  \\ 
all & & 81 & 79 & \textbf{84} & 83 & \\ \midrule
bashkir & \multirow{5}{*}{turkmen} &  82 &  76 &  82 &  88 & \multirow{5}{*}{80$\pm$4} \\ 
arabic &  &  64 &  66 & 84 &  80 \\ 
turkish & &  82 &  88 &  90 &  \textbf{92}\\ 
uzbek & &  66 &  74 & 86 &  78 &\\ 
all & & \textbf{92} & 90 & 84 & 88 & \\ \midrule
\ifaclfinal
estonian & \multirow{4}{*}{votic} &  12 &  17 &  23 &  27 &\multirow{4}{*}{26.3$\pm$2.1} \\ 
finnish &  &  24 &  20 &  26 & 28 \\ 
hungarian & &  10 &  10 &  24 &  \textbf{30} \\
all & & 17 & 20 & 28 & 29 & \\ \midrule
dutch & \multirow{2}{*}[-.6em]{west} &  36 &  39 &  44 &  \textbf{49} & \multirow{4}{*}{47$\pm$1}  \\ 
english &  &  36 &  25 &  45 &  43 \\
danish & \multirow{2}{*}[.6em]{frisian} &  33 &  33 &  42 &  43  \\ 
all & & 40 & 38 & 43 & 45 & \\ \midrule
danish & \multirow{4}{*}{yiddish} &  50 &  54 &  55 & 56 & \multirow{4}{*}{55.3$\pm$0.6}  \\
dutch &  &  49 &  50 & 56 &  55 & \\
german & &  53 &  54 &  \textbf{57} &  54  \\
all & & 55 & 55 & 55 & 54 & \\ 
\midrule
\fi
\multicolumn{2}{c}{Average (both parts)} & 49.00 & 48.48 & 59.36 & 60.18 & 57.9\\
\bottomrule
\end{tabular}
\caption{Multiple transfer language results part 2.}
\label{tab:results_multiple_two}
\end{table}

==> results.tex <==
\begin{table*}
\centering
\small
\begin{tabular}{cccccccc}
\toprule
L1 & L2 & Simple & +L & +hall & +hall +L & hallonly & Best-hallonly \\ \hline
turkish & \multirow{5}{*}{azeri} & 81 &  77 &  80 &  81 &  68 & 13 \\ 
persian & &  35 &  43 &  74 &  69 &  66 & 8 \\ 
bashkir & &  37 &  39 &  66 &  67 &  66 & 1 \\
uzbek & &  27 &  35 &  74 &  70 &  67 & 7 \\ 
all & & 84 & 71 & 83 & \textbf{87}\\ \hline
urdu & \multirow{5}{*}{bengali} &  32 &  22 &  66 &  67 &  \textbf{69} & 0 \\
sanskrit & &  34 &  28 &  66 &  65 &  65 & 1 \\ 
hindi & &  39 &  42 &  67 &  65 &  60 & 7 \\ 
greek & &  32 &  26 &  65 &  67 &  61 & 6 \\ 
all & & 39 & 40 & 64  &   62 \\ \hline
welsh & \multirow{4}{*}{breton} &  44 &  45 &  83 &  86 &  81 & 5 \\ 
irish & &  28 &  42 &  80 &  \textbf{88} &  78 & 10 \\
albanian & &  33 &  39 &  78 &  81 &  76 & 5 \\
all & & 52 & 45 & 81 & 82 & \\ \hline
hebrew & \multirow{3}{*}{classical-syriac} &  86 &  85 & 95 & 95 &  94 & 1 \\ 
arabic & &  83 &  82 &  92 & 95 &  94 & 1 \\ 
all & & 87 & 85 & 95 & \textbf{96} & \\ \hline
irish & \multirow{3}{*}{cornish} &  8 &  14 & 14 &  10 & 14 & 0 \\ 
welsh & &  16 &  \textbf{18} &  \textbf{18} &  14 &  14 & 4 \\
all & & 12 & 6 & 12 & 14 & \\ \hline
turkish & \multirow{4}{*}{crimean-tatar} &  87 &  80 &  85 &  \textbf{89} &  72 & 17 \\ 
bashkir & &  59 &  60 & 70 &  69 & 70 & 0 \\ 
uzbek & &  6 &  6 & 72 &  67 &  72 & 0 \\ 
all & & 82 & 81 & 88 & 80 & \\ \hline
latin & czech &  15 &  26 &  71.4 &  68 &  \textbf{77.4} & 0 \\ \hline
spanish & \multirow{3}{*}{friulian} &  50 &  50 &  81 &  \textbf{83} &  76 & 7 \\ 
italian & &  51 &  50 &  78 &  77 & 81 & 0 \\ 
all & & 64 & 58 & 78 & \textbf{83} & \\ \hline
bengali & greek &  12.4 &  6.4 &  70.5 &  70.6 &  \textbf{71.6} & 0 \\ \hline
finnish & \multirow{4}{*}{ingrian} &  18 &  16 &  14 & 20 &  16 & 4 \\ 
hungarian & &  8 &  12 &  12 & 18 &  16 & 2 \\ 
estonian & &  12 &  12 &  12 & 18 &  12 & 6 \\ 
all & & 18 & \textbf{24} & 16 & 16 & \\ \hline
sorani & irish &  10.3 &  8.6 &  \textbf{66.3} &  64.6 &  65.6 & 0.7 \\ \hline
adyghe & \multirow{3}{*}{kabardian} &  92 &  92 &  93 &  \textbf{96} &  95 & 1 \\ 
armenian & &  78 &  77 &  86 &  80 & 87 & 0 \\ 
all & & 95 & 91 & 93 & 90 & \\ \hline
finnish & \multirow{4}{*}{karelian} &  44 &  40 & 48 &  46 &  42 & 6 \\ 
hungarian & &  32 &  36 & 48 &  42 &  42 & 6 \\ 
estonian & &  32 &  32 &  44 & 48 &  44 & 4 \\
all & & 40 & 36 & 44 & \textbf{54} & \\ \hline
basque & \multirow{5}{*}{kashubian} &  36 &  30 &  70 &  76 &  72 & 4 \\ 
slovak & &  48 &  52 &  74 & 76 & 76 & 0 \\ 
czech & &  44 &  54 & 78 &  66 &  72 & 6 \\ 
polish & &  66 &  78 &  78 &  \textbf{80} &  76 & 4 \\ 
all & & 70 & 72 & 78 & \textbf{80} & \\ \hline
turkish & \multirow{4}{*}{kazakh} &  \textbf{86} &  80 &  74 &  66 &  70 & 16 \\ 
bashkir &  &  68 & 84 &  74 &  70 &  74 & 10 \\ 
uzbek & &  66 &  60 & 78 &  70 &  76 & 2 \\ 
all & & 76 & 78 & 80 & 78 & \\ \hline
bashkir & \multirow{4}{*}{khakas} &  82 &  78 &  80 & 84 &  68 & 16 \\ 
uzbek & & 84 &  80 &  72 &  76 &  72 & 12 \\ 
turkish & & 90 & 90 &  80 &  82 &  80 & 10 \\ 
all & & 84 & \textbf{92} & 86 & 84 & \\ \hline
italian & ladin &  48 &  54 &  \textbf{74} &  \textbf{74} &  \textbf{74} & 0 \\ \hline
czech & \multirow{3}{*}{latin} &  5.4 &  5 &  20.6 & 42 &  40.8 & 1.2 \\ 
romanian & &  7.9 &  9 &  18.8 &  41.3 & 42.9 & 0 \\ 
all & & 3.6 &  7.7 & 40.1 &  \textbf{44.1} \\ \hline
latvian & lithuanian &  7.1 &  13.2 &  48.4 &  48.4 &  \textbf{50.5} & 0 \\ \hline
estonian & \multirow{3}{*}{livonian} &  22 &  22 & 35 &  34 &  33 & 2 \\ 
hungarian & &  23 &  25 & 35 &  33 &  34 & 1 \\ 
finnish &  &  25 &  21 &  34 & 35 &  32 & 3 \\ 
all & & 21 & 20 & \textbf{36} & \textbf{36} \\ \hline
italian & \multirow{4}{*}{maltese} &  34 &  25 &  48 &  42 &  \textbf{52} & 0 \\ 
arabic & &  18 &  26 & 41 &  38 & 41 & 0 \\ 
hebrew & &  20 &  21 & 47 &  45 &  44 & 3 \\ 
all & & 29 & 28 & 40 & 46 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}
\centering
\small
\begin{tabular}{cccccccc}
\toprule
danish & \multirow{4}{*}{middle-high-german} &  68 &  58 &  78 &  80 &  70 & 10 \\ 
dutch &  &  70 &  62 &  74 & 82 &  78 & 4 \\ 
german & &  72 &  68 &  \textbf{86} &  82 &  82 & 4 \\
all & & 70 & 70 & 84 & 78 \\ \hline
dutch & \multirow{4}{*}{middle-low-german} &  36 & 42 &  32 &  36 &  36 & 6 \\
german &  &  \textbf{46} &  26 &  32 &  38 &  40 & 6 \\ 
danish & &  30 &  24 &  30 &  30 & 34 & 0 \\
all & & 32 & 42 & 36 & 38 & \\ \hline
english & murrinhpatha &  \textbf{36} &  2 &  6 &  20 &  20 & 16 \\ \hline
italian & neapolitan &  70 &  70 &  83 &  83 &  \textbf{84} & 0 \\ \hline
danish & \multirow{4}{*}{north-frisian} &  18 &  25 &  44 &  46 &  43 & 3 \\ 
dutch &  &  28 &  22 &  \textbf{47} &  46 &  44 & 3 \\
english &  &  22 &  26 &  \textbf{47} &  42 &  42 & 5 \\ 
all & & 23 & 25 & 43 & 46 & \\ \hline
asturian & \multirow{4}{*}{occitan} &  58 &  49 &  77 &  74 & 78 & 0 \\ 
spanish & &  47 &  55 &  78 &  76 &  \textbf{82} & 0 \\ 
french & &  41 &  52 & 80& 80 &  75 & 5 \\ 
all & & 52 & 61 & 78 & 80 & \\ \hline
russian & \multirow{4}{*}{old-church-slavonic} &  40 &  39 &  39 &  \textbf{64} &  56 & 8 \\ 
polish &  &  41 &  41 & 59 &  58 &  59 & 0 \\ 
bulgarian &  &  38 &  42 &  44 &  56 & 57 & 0 \\
all & & 41 & 42 & \textbf{64} & 56 & \\ \hline
urdu & old-english &  13.8 &  8.5 &  43.4 &  40.4 &  \textbf{44.3} & 0 \\ \hline
irish & \multirow{4}{*}{old-irish} &  2 &  4 &  \textbf{12} &  2 &  6 & 6 \\ 
belarusian & &  10 & 10 & 10 &  6 &  8 & 2 \\
welsh &  &  4 &  6 & 10 &  6 &  4 & 6 \\ 
all & & 4 & 4 & 8 & 6 & \\ \hline
slovene & old-saxon &  10.7 &  14.7 &  \textbf{52.3} &  50.5 &  50.5 & 1.8 \\ \hline
sanskrit & \multirow{3}{*}{pashto} &  10 &  6 &  46 &  44 &  \textbf{49} & 0 \\ 
persian & &  26 &  18 &  39 & 48 &  44 & 4 \\ 
all & & 19 & 20 & 46 & \textbf{49} & \\ \hline
russian & portuguese &  34.5 &  22.2 &  \textbf{88.8} &  88.4 &  87.7 & 1.1 \\ \hline
swahili & quechua &  4.2 &  2.8 &  \textbf{92.1} &  91.6 &  91.6 & 0.5 \\ \hline
portuguese & russian &  25.6 &  17.5 &  \textbf{76.3} &  74.6 &  74.3 & 2 \\ \hline
welsh & \multirow{4}{*}{scottish-gaelic} &  46 &  34 &  64 & 64 &  56 & 8 \\ 
irish & &  58 &  62 &  \textbf{68} &  66 &  58 & 10 \\ 
latvian &  &  58 &  36 &  58 & 66 &  60 & 6 \\ 
all & & 60 & 64 & 62 & 66 & \\ \hline
kurmanji & sorani &  6.2 &  3.6 &  \textbf{69} &  64.3 &  66.7 & 2.3 \\ \hline
zulu & swahili &  46 &  52 &  \textbf{81} &  80 &  76 & 5 \\ \hline
bashkir & \multirow{4}{*}{tatar} &  67 &  64 &  73 &  69 &  72 & 1 \\ 
uzbek &  &  25 &  15 &  47 & 72 &  69 & 3 \\ 
turkish &  &  81 &  79 &  82 &  75 &  78 & 4 \\ 
all & & 81 & 79 & \textbf{84} & 83 & \\ \hline
kannada & telugu &  76 &  72 &  \textbf{94} &  90 &  \textbf{94} & 0 \\ \hline
bashkir & \multirow{5}{*}{turkmen} &  82 &  76 &  82 &  88 &  82 & 6 \\ 
arabic &  &  64 &  66 & 84 &  80 &  74 & 10 \\ 
turkish & &  82 &  88 &  90 &  \textbf{92} &  82 & 10 \\ 
uzbek & &  36 &  44 & 86 &  78 &  82 & 4 \\ 
all & & \textbf{92} & 90 & 84 & 88 & \\ \hline
estonian & \multirow{4}{*}{votic} &  12 &  17 &  23 &  27 & 27 & 0 \\ 
finnish &  &  24 &  20 &  26 & 28 & 28 & 0 \\ 
hungarian & &  10 &  10 &  24 &  \textbf{30} &  24 & 6 \\
all & & 17 & 20 & 28 & 29 & \\ \hline
dutch & \multirow{4}{*}{west-frisian} &  36 &  39 &  44 &  \textbf{49} &  48 & 1 \\ 
english &  &  36 &  25 &  45 &  43 & 47 & 0 \\
danish & &  33 &  33 &  42 &  43 & 46 & 0 \\ 
all & & 40 & 38 & 43 & 45 & \\ \hline
danish & \multirow{4}{*}{yiddish} &  10 &  14 &  15 & 16 &  15 & 1 \\
dutch &  &  9 &  10 & 16 &  15 & 16 & 0 \\
german & &  13 &  14 &  \textbf{17} &  14 &  15 & 2 \\
all & & 15 & 15 & 15 & 14 & \\ 
\midrule
Average & & 39.14 & 38.345 & 57.65 & 58.47 & 57.48 & 3.9 \\
\end{tabular}
\label{tab:results}
\caption{All Results}
\end{table*}
